Structured Regularization of Functional Map Computations

We consider the problem of non-rigid shape matching using the functional map framework. Specifically, we analyze a commonly used approach for regularizing functional maps, which consists in penalizing the failure of the unknown map to commute with the Laplace-Beltrami operators on the source and target shapes. We show that this approach has certain undesirable fundamental theoretical limitations, and can be undefined even for trivial maps in the smooth setting. Instead we propose a novel, theoretically well-justified approach for regularizing functional maps, by using the notion of the resolvent of the Laplacian operator. In addition, we provide a natural one-parameter family of regularizers, that can be easily tuned depending on the expected approximate isometry of the input shape pair. We show on a wide range of shape correspondence scenarios that our novel regularization leads to an improvement in the quality of the estimated functional, and ultimately pointwise correspondences before and after commonly-used refinement techniques.

==> backup.tex <==

%---------------------------------------------------------------------------------- 
% the old version of the summary curves
%\subsection{Summary error curves}
%\begin{figure*}[!ht]
%\centering
%\input{figures_tex/summaryCurve_norm_faust100.tex}
%\input{figures_tex/summaryCurve_norm_faust200.tex}
%\input{figures_tex/summaryCurve_norm_faust300.tex}
%\input{figures_tex/summaryCurve_norm_tosca.tex}
%\caption{normalized dataset, direct measurement}
%\label{fig:res:summary:original:direct}
%\end{figure*}

% the relative improvement table
%\begin{table}[]
%\centering
%\begin{tabular}{cccc}
%\hline
%\multirow{2}{*}{Dataset} & \multicolumn{3}{c}{relative improvement (\%)} \\ \cline{2-4} 
% & Initialization & +ICP & +BCICP \\ \hline
%FAUST1 & 37.97 & 31.10 & 3.81 \\
%FAUST2 & 45.12 & 52.20 & 31.01 \\
%FAUST3 & 36.37 & 43.17 & 15.78 \\
%TOSCA & 34.04 & 42.38 & 24.79 \\ \hline
%\end{tabular}
%\caption{relative improvement on the average direct error over the best of slanted or the standard}
%\end{table}

==> sec_results_old.tex <==
\section{Results}
\label{sec:results}
%-----------------------------------------------------------------------------------------
\input{tables/tb_AveErr_Summary_new.tex}

\begin{figure*}[!ht]
\centering
\includegraphics[width = 2\columnwidth]{figures/SummaryCurve_perVtx.png}
\caption{Per-vertex measurement. For each dataset, we compare the quality of the functional maps with the old (blue curves) and the new (red curves) mask with the same set of parameters. The gray curves are the results of old mask using the parameters in \cite{ren2018continuous}, and they are included to show that the parameters we choose are reasonable to make a fair comparison. We can compare the new mask (red) to the old mask (blue) in three settings: comparing the initialization directly (solid lines), comparing the initialization with ICP refinement (dashed lines), and with the BCICP refinement (dotted lines). Specifically, these curves are measured on 200 FAUST isometric pairs, 400 FAUST non-isometric pairs, 568 TOSCA isometric pairs, and 190 TOSCA non-isometric pairs.}
\label{fig:summary:perVtx}
%\vskip-2mm
\end{figure*}

\begin{figure*}[!ht]
\centering
\includegraphics[width = 2\columnwidth]{figures/SummaryCurve_perMap.png}
\caption{Per-map measurement. Similar to Fig.~\ref{fig:summary:perVtx}, here we show the per-map measurement of the point-wise maps on the same datasets.}
\label{fig:summary:perMap}
%\vskip-2mm
\end{figure*}

\begin{figure*}[!ht]
\centering
\includegraphics[width = 2\columnwidth]{figures/SummaryCurve_direct.png}
\caption{Direct measurement. Here we show the direct error of the point-wise maps.}
\label{fig:summary:direct}
%\vskip-2mm
\end{figure*}
%-----------------------------------------------------------------------------------------

We tested the proposed approach using a simple MATLAB-based implementation. Here we first describe the benchmark datasets and the baseline methods. 

\myparagraph{Datasets}
We use the standard benchmark datasets for evaluation: FAUST~\cite{Bogo:CVPR:2014} and TOSCA~\cite{tosca}. We use the LRVD algorithm~\cite{yan2014low} to remesh the models so that they do not share the same connectivity. For each of the dataset, we split them into two categories: isometric and non-isometric.
\begin{itemize}
    \item \textbf{FAUST}: The FAUST dataset contains meshes of ten different humans in ten different poses each.
    \begin{itemize}
        \item \textbf{Isometric}: we randomly selected~100 isometric shape pairs stemming from the same person.
        \item \textbf{Non-Isometric}: we randomly selected~200 non-isometric shape pairs, consisting of 100 pairs of meshes stemming from different person but with the same pose, and 100 pairs of meshes stemming from different person with different pose.
    \end{itemize}
    \item \textbf{TOSCA}: The TOSCA dataset contains 80 meshes of humans and animals in 9 categories.
    \begin{itemize}
        \item \textbf{Isometric}: we randomly selected 284 isometric shape pairs, consisting of:  66 pairs of Victoria, 60 pairs of Michael, 55 pairs of cats, 36 pairs of dogs, 28 pairs of horse, 21 pairs of David, 15 pairs of centaurs, and 3 pairs of wolves.
        \item \textbf{Non-Isometric}: we picked 60 pairs of gorillas and Victoria, and 35 pairs of gorillas and Michael, with dense human-verified ground truth correspondences.
    \end{itemize}
\end{itemize}
Note that for each of the datasets, we evaluated the point-wise maps in both directions, for each pair.

\myparagraph{Baselines}
To evaluate our new regularizer, we consider the following three settings:
\begin{itemize}
    \item \textbf{Initialization}. The Wave kernel signatures (WKS) are used to construct $E_{\text{desc}}, E_{\text{mult}}$ and $E_{\text{orient}}$ in Eq. \eqref{eq:energy:complete}. Then we optimize the functional map w.r.t. the energy defined in Eq.~\eqref{eq:energy:complete} using our resolvent-based commutativity term and compare it to the original Laplacian-commutativity term (the old mask).
    \item \textbf{With ICP refinement}. We use ICP~\cite{ovsjanikov2012functional} to refine the computed functional maps.
    \item \textbf{With BCICP refinement}. We use the recently proposed BCICP~\cite{ren2018continuous} to refine the computed functional and pointwise maps, using the open-source implementation and default parameters provided by the authors.
\end{itemize}

\myparagraph{Measurement}
In our experiments, we measured the quality of the functional maps and the recovered point-wise maps:
\begin{itemize}
    \item \textbf{Point-wise maps}. Since most shapes contain left-right symmetries, which are indinstinguishable for intrinsic methods, in each dataset, we considered both the ground-truth direct and symmetric correspondences are given. To measure the accuracy of a computed map, we used the following measures:
	\begin{itemize}
	\item \textbf{per-vertex error}: for each vertex we accept the ground-truth direct and symmetric correspondences and take the minimum as the error of this vertex.
	\item \textbf{per-map error}: we compute the average per-vertex error to the direct map and the average per-vertex error to the symmetric map and take the minimum of these two metrics.
	\item \textbf{direct error}: we compute the average per-vertex error to the direct ground-truth correspondences only.
	\end{itemize}
    \item \textbf{Functional maps}. We can evaluate a functional map by the quality of its recovered point-wise map, or by measuring the penalty from a given mask. Specifically, for a given functional map $\matr{C}$ and a  mask matrix $\matr{M}$, we can measure the total penalty as 
    $\Vert\,\matr{M} \odot \matr{C} \Vert_F^2$
    where $\odot$ is the element-wise matrix product. 
\end{itemize}

%-------------------------------------------------------------------------------------------------------------------------------------
\subsection{Evaluation on shape matching}
%-------------------------------------------------------------------------------------------------------------------------------------


\begin{figure}[!t]
\centering
\includegraphics[width = 0.98\columnwidth]{figures/egINI_tosca_Iso_new.png}
\caption{Here we show the initial maps optimized with the old and the new mask on a pair from the TOSCA isometric dataset. We can see that using the new mask achieves a more accurate map on the legs compared to the result with the old mask.}
\label{fig:eg:INI:tosca_iso1}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width = 0.98\columnwidth]{figures/egINI_tosca_Iso_lines.png}
\caption{Similar to Fig.~\ref{fig:eg:INI:tosca_iso1}, we show another TOSCA isometric pair where the new mask achieves better correspondences around the left arm.}
\label{fig:eg:INI:tosca_iso2}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[width = 0.98\columnwidth]{figures/egICP_faust.png}
\caption{Maps of a FAUST non-isometric pair are refined with ICP and visualized via texture transfer. We can see that the map optimized using the new mask has much less distortion in the front area after the ICP refinement.}
\label{fig:eg:ICP:faust}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[width = 0.98\columnwidth]{figures/egBCICP_tosca_nonIso.png}
\caption{Improvement of the maps of a TOSCA non-isometric pair refined with BCICP. For the initialization optimized using the old mask, the refinement step fails to correct the errors of mapping the front to the back. However, with a better initialization optimized with the new mask regularizer, the BCICP refinement can benefit from it and produce a more accurate point-wise map.}
\label{fig:eg:BCICP:tosca_noniso}
\end{figure}

%\begin{figure}[!ht]
%\centering
%\includegraphics[width = 0.98\columnwidth]{figures/egAll_faust.png}
%\caption{For a FAUST non-isometric pair, we compare the results using the old and %the new mask before and after the refinement techniques. We can see that there is a %consistent improvement coming from the new mask.}
%\label{fig:eg:all:faust}
%\end{figure}

In our experiments, we tested the new mask regularizer on the described four datasets (FAUST/TOSCA: isometric and non-isometric) w.r.t. three settings: the initialization, with ICP refinement, and with BCICP refinement. The average geodesic errors of the point-wise map w.r.t. three different measurements (per-vertex, per-map and direct), and the relative improvement over the old  regularizer are summarized in Table~\ref{tb:res:aveErr_summary}.~\cref{fig:summary:perVtx,fig:summary:perMap,fig:summary:direct} show the corresponding cumulative curves of the percentage of matches that have error smaller than a threshold.

Specifically, when comparing the initialization optimized with the old mask regularizer, the results of using the new mask achieved 28.8\% improvement on FAUST isometric dataset, 24.7\% on FAUST non-isometric dataset, 15.7\% on TOSCA isometric dataset, and 21.0\% on TOSCA non-isometric dataset with respect to the \textbf{direct} error. Comparing the results with ICP refinement, the new mask achieved 17.8\%, 14.4\%, 15.1\%, and 16.4\% improvement on the four datasets respectively w.r.t. the direct error. As for the results with BCICP refinement, the new mask achieved 12.4\%, 8.29\%, 3.32\%, and 26.1\% improvement respectively. 


Fig.~\ref{fig:eg:INI:tosca_iso1} and~\ref{fig:eg:INI:tosca_iso2} show two TOSCA isometric pairs, where the functional maps are optimized for with the old and the new mask respectively, and the point-wise maps are obtained without any refinement.
Fig.~\ref{fig:eg:ICP:faust} shows an example pair of FAUST non-isometric dataset after ICP refinement visualized via texture transfer.
Fig.~\ref{fig:eg:BCICP:tosca_noniso} shows an example pair of TOSCA non-isometric dataset, where the point-wise maps after BCICP refinement are visualized.
%Fig.~\ref{fig:eg:all:faust} shows the point-wise maps of an FAUST non-isometric pair before and after the ICP, BCICP refinement.



\begin{figure}[!t]
\centering
\includegraphics[width = 0.98\columnwidth]{figures/Average_GroudTruth_fMap.png}
\caption{Average ground-truth functional map. For each of the datasets, we average the squared ground-truth functional map over all the shape pairs.}
\label{fig:res:ave_gt_fmap}
\vskip-4mm
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width = 0.98\columnwidth]{figures/allMask_old.png}
\caption{Average old mask. Here we show the average of the old masks over all the shape pairs for each dataset.}
\label{fig:res:ave_old_mask}
\vskip-4mm
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width = 0.98\columnwidth]{figures/allMask_new.png}
\caption{Average mask with $\gamma = 0.4$ for the FAUST isometric, non-isometric, and TOSCA isometric dataset; $\gamma = 0.2$ for the TOSCA non-isometric dataset.}
\label{fig:res:ave_new_mask}
\end{figure}
%-------------------------------------------------------------------------------------------------------------------------------------
\subsection{Justification of the new mask}
%-------------------------------------------------------------------------------------------------------------------------------------

In order to see how well our new mask fits with the ground truth data, in Fig.~\ref{fig:res:ave_gt_fmap} we show the average functional map constructed from the ground-truth correspondences using 250 eigen-functions. 
Fig.~\ref{fig:res:ave_old_mask} shows the average old mask over all the shape pairs in each dataset, and Fig.~\ref{fig:res:ave_new_mask} shows the average new mask, where the masks are normalized to Frobenius-norm 1. Visually, we can see the structure of the new mask is more consistent with the funnel structure shown in Fig.~\ref{fig:res:ave_gt_fmap}. Specifically, for the region of ground-truth functional map with smaller values (white regions in Fig.~\ref{fig:res:ave_gt_fmap}), there is more penalty added by the new mask (red regions in Fig.~\ref{fig:res:ave_new_mask}).
To justify that the new mask is a better regularizer than the old one, we also measure the penalty of the masks added to the ground-truth functional maps. Fig.~\ref{fig:res:mask_gtFmap} shows that our new regularizer (red curve) penalizes the ground-truth functional maps less than the old one (blue curve). 


\begin{figure}[!t]
\centering
\includegraphics[width = 0.45\columnwidth]{figures/energy_mask_gtFmap_faust.png}
\includegraphics[width = 0.45\columnwidth]{figures/energy_mask_gtFmap_tosca.png}
\caption{Comparing the penalty on the ground-truth functional map with the old and the new mask on two datasets. All  masks are normalized to Frobenius-norm 1.}
\label{fig:res:mask_gtFmap}
\end{figure}

% Fig.~\ref{fig:res:egMask:tosca_iso} shows an example pair from the TOSCA isometric dataset, where the old and new mask are visualized on the top, and the corresponding recovered point-wise map are visualized on the bottom. We can see that the new mask has a similar funnel pattern as the ground-truth functional map shown in Fig.~\ref{fig:res:ave_gt_fmap}, and the corresponding point-wise map has a higher quality compared to the old mask.

% \begin{figure}[!t]
% \centering
% \includegraphics[width = 0.98\columnwidth]{figures/example_mask_tosca.png}
% \caption{An example isometric pair from the TOSCA dataset.}
% \label{fig:res:egMask:tosca_iso}
% \end{figure}


\begin{figure}[!ht]
\centering
\includegraphics[width = 0.98\columnwidth]{figures/correlation_between_errorAndEnergy.png}
\caption{Correlation between the mask penalty on a functional map and the accuracy of the corresponding point-wise map. For a TOSCA isometric pair, we sample 3k functional maps with different quality (normalized to the same scale). We measure the element-wise product between the functional map and the old/new mask, as an indicator of the quality of the functional map. We also measure the average geodesic error (w.r.t. the direct measurement) of the recovered point-wise map of the corresponding functional map. The correlation between the functional map penalty and the point-wise map quality is visualized as a scatter plot with 3k samples. Compared to the old mask, the new mask penalizes a functional map with a good underlying point-wise map less and a functional map with a bad underlying point-wise map more heavily.}
\label{fig:res:correlation}
\end{figure}

Fig.~\ref{fig:res:correlation} shows the correlation between the regulizer (mask) penalty on a functional map and the accuracy of the corresponding point-wise map. In this experiment, we generated 3000 different random point-to-point maps, converted them to a functional representation and measured the penalty of the mask vs. the average geodesic error computed from the pointwise maps. We can observe that, compared to the old mask, the new mask induces a lower penalty on functional maps with a good quality (i.e., smaller average geodesic error), and penalizes a functional map with larger error more heavily. This further confirms that using our new regularizer is more likely to produce a better functional, and ultimately better pointwise map.


\begin{figure}[!t]
\centering
\includegraphics[width = 0.98\columnwidth]{figures/diff_dimension.png}
\caption{
\jing{
Comparison to the old mask with high frequencies. For a test shape pair, we fix the input corresponding descriptors and optimize for different size of functional maps ranging from 30 to 250. Then average per-vertex error w.r.t. different functional map size and different masks are reported. The blue lines correspond to the old mask, and the red lineds correspond to our new mask. The solid lines are the results of the initialization, and the dashed lines are the results refined by ICP for 10 iterations.}
}
\label{fig:res:diff_dimension}
\end{figure}

\jing{
Fig.~\ref{fig:res:diff_dimension} shows a comparison between the old and our new mask with higher frequencies included into the functional map computation. Specifically, we fix the input descriptors for a test pair, and optimize for functional maps with different sizes. Note that, with a given number of input descriptors, the constraints for the functional map computation is fixed. If we increase the functional map size, the number of variables gets increased as well. Therefore, in this case, we rely more heavily on the regularizers to produce a good function map. From Fig.~\ref{fig:res:diff_dimension}, we can see that the old mask (blue lines) fails to regularize the functional map with large size: the accuracy gets worse when the size gets larger. However, the new mask (red lines) are more stable than the old mask when the computation gets less constrained with a larger number of variables. This aligns well with the theory justification, that the old mask makes less sense than our new mask when higher frequencies are included.
}


%-------------------------------------------------------------------------------------------------------------------------------------
\subsection{Comparison to Heat Mask}
%-------------------------------------------------------------------------------------------------------------------------------------
\begin{figure}[!ht]
\centering
\includegraphics[width = 0.98\columnwidth]{figures/heatMask_diffGamma.png}
\caption{Visualization of the heat mask with different time-scale parameter $T$.}
\label{fig:res:heatMask}
\end{figure}


\begin{figure}[!ht]
\centering
\includegraphics[width = 0.98\columnwidth]{figures/heatMask_performance.png}
\caption{Changing $T$ of the heat mask. Here we test the performance of the heat mask (yellow curve) with different $T$ and report the average direct error of~50 random FAUST isometric shape pairs. The average error of the old mask (blue dashed line) and the average error the new mask with $\gamma = 0.4$ (red dashed line) are included for comparison. All the masks (old, new, and heat with different parameters) are normalized with Frobenius-norm 1 for a fair comparison. The visualization of the heat mask with the smallest error is given on the right.}
\label{fig:res:heatMask:curve}
\end{figure}

Besides our resolvent-based commutativity term, another natural bounded option would be to use the commutativity with the \emph{heat} operators, which are also bounded linear functional operators, which can act as regularizers on functional maps. This would lead to the following mask matrix:
\begin{equation}
\matr{M}_{heat}(i,j) = \exp(-T \Lambda_2(i)) - \exp(-T \Lambda_1(j)),
\end{equation}
where $T$ is the scalar time parameter. Fig.~\ref{fig:res:heatMask} visualizes the heat mask with different values of $T$ on an isometric shape pair. In Fig.~\ref{fig:res:heatMask:curve} we compared the performance of the heat mask with different values of $T$ ranging from $10^{-3}$ to 500 on FAUST isometric shape pairs. We can see that, in the range $[1, 50]$, the heat mask has a better performance than the old mask. When $T = 7$, it gives the best performance among the tested values. The heat mask with $T = 7$ (in Fig.~\ref{fig:res:heatMask:curve}) has a similar structure as our new mask with $\gamma = 0.4$, but still does not achieve the quality of the results we obtain with the new mask based on the resolvent operators.


%-------------------------------------------------------------------------------------------------------------------------------------
\subsection{Comparison to Slanted Mask}
%-------------------------------------------------------------------------------------------------------------------------------------
\begin{figure}[!ht]
\centering
\includegraphics[width = 0.98\columnwidth]{figures/slantMask_examples.png}
\caption{
\jing{
Visualization of the slanted mask with different parameter $\eta$.
}
}
\label{fig:res:slantMask}
\end{figure}

\begin{figure}[!ht]
\centering
\includegraphics[width = 0.98\columnwidth]{figures/slantMask_curve.png}
\caption{
\jing{
Change $\eta$ of the slanted Mask.
}
}
\label{fig:res:slantMask:curve}
\end{figure}


\jing{
In~\cite{rodola2017partial}, a slanted-diagonal structure of a functional is proposed for regularization. The weight matrix $\matr{W}$ is defined as:
$$w_{ij} = \exp{\big(-\eta \sqrt{i^2 + j^2}\big)}\big\Vert \frac{\vec{n}}{\Vert \vec{n} \Vert} \times \big((i,j)\tran - \vec{p}\big)\big\Vert$$

where $\vec{p} = (1,1)\tran$ is the matrix origin, and $\vec{n} = (1,r/k)\tran$ is the line direction with slope $r/k$, where $r$ is the estimated rank of the functional map, and $k$ is the size of the square functional map. 

This weight matrix proposed in~\cite{rodola2017partial} is applied to partial shape matching setting, which can also be used as a penalty mask and compared with ours in the general shape matching setting. 
Fig.~\ref{fig:res:slantMask} visualizes the slanted mask with different values of $\eta$.
In~Fig.~\ref{fig:res:slantMask:curve}, we compared the performance of the slanted mask with different $\eta$ ranging from 0.005 to 0.5 on 100 TOSCA isometric shape pairs. We can see that, when $\eta = 0.09$, it achieves the best performance over the tested values and the corresponding slanted mask is visualized on the right. The best slanted mask does have a funnel structure, which helps to improve the performance over the old mask. However, our new mask based on the resolvent operators with theoretical justification still outperforms the heuristic slanted mask with different $\eta$.

}




%-------------------------------------------------------------------------------------------------------------------------------------
\subsection{Parameters \& Performance}
%-------------------------------------------------------------------------------------------------------------------------------------
\begin{figure}[!ht]
\centering
%\includegraphics[width = 0.98\columnwidth]{figures/tosca_diffWeight.png}
\includegraphics[width = 0.98\columnwidth]{figures/tosca_diffWeight_new.png}
\caption{We change the weight $\alpha_3$ of the regularizer term in Eq.~\eqref{eq:energy:complete} and compare the results with the old and new mask to verify that the new mask improves the performance in general. Specifically, for random 100 TOSCA isometric pairs, we test 50 different values of the weight from 0 to 1 while keeping the other weights fixed. Both the new and the old mask are normalized to the same scale. We report the average geodesic error over all the pairs.}
\label{fig:res:diffWeight:tosca}
\end{figure}

In our experiments, there are mainly two sets of parameters: (1) the weights $\alpha_i$ for different terms; (2) the parameter $\gamma$ for the mask structure in Eq. \eqref{eq:res_penalty}.
For each of the datasets, the parameters are fixed for all the pairs in this dataset. In particular we set the parameters $\alpha_1, \alpha_2$ and $\alpha_4$ in a uniform way regardless of the choice of regularizer.
% Specifically, instead of fixing $\alpha_i$ directly, we would like to fix the relative weight of each term, i.e., $\beta_i = \alpha_i E_i (\matr{I})$ where $\matr{I}$ is an identity matrix, as an initial guess for the functional map. With a given set of $\beta_i$ for a specific dataset, we can compute the $\alpha_i = \frac{\beta_i}{E_i(\matr{I})}$ for each tested pair, and they have different values since the energy function $E_i$ constructed from shape descriptors are different from pair to pair. This is a better way to set the parameters, since in this case, the relative weights between different terms are the same across the whole dataset. In our experiments, for FAUST isometric and non-isometric datasets, we set $\beta_1 = 2,\beta_2 = 0.1, \beta_3 = 0.008, \beta_4 = 1$; for TOSCA isometric dataset, we set $\beta_1 = 1, \beta_2 = 0.1, \beta_3 = 0.007, \beta_4 = 0.2$; for TOSCA non-isometric dataset, we set $\beta_1 = 0.5, \beta_2 = 0.01, \beta_3 = 0.2, \beta_4 = 0.2$. 
%The choices of these parameters are computed from the $\alpha_i$ used in~\cite{ren2018continuous}. 
For the FAUST isometric and non-isometric datasets, and the TOSCA isometric dataset, we set $\gamma = 0.4$ to construct the mask. As for the most challenging dataset, TOSCA non-isometric dataset, we used a regularizer consisting of two terms with $\gamma=1$ and $\gamma=0.2$ respectively.


\begin{figure}[!t]
\centering
\includegraphics[width = 1.0\columnwidth]{figures/diffWeight_example.png}
\caption{We illustrate the effect of changing the weight of the regularizer term $\alpha_3$.}
\label{fig:res:diffWeight:example}
\end{figure}

\begin{figure}[!t]
\centering
%\includegraphics[width = 0.98\columnwidth]{figures/faust_diffGamma.png}
\includegraphics[width = 0.98\columnwidth]{figures/diffGamma_all_new.png}
\caption{Changing $\gamma$ of the new mask defined in Eq.~\eqref{eq:mtd:def:mask_new}. For each of the datasets, we randomly select 50 shape pairs, then change the $\gamma$ from 0.05 to 1 and report the corresponding average direct error over all the pairs. We can see that the non-isometric dataset prefers a smaller $\gamma$, which is consistent with the structure of the ground-truth functional map in Fig.~\ref{fig:res:ave_gt_fmap}.}
\label{fig:res:diffGamma:faust}
\end{figure}

Fig.~\ref{fig:res:diffWeight:tosca} shows the performance of the old and new mask with different weight $\alpha_3$ in Eq.~\eqref{eq:energy:complete} on the TOSCA isometric dataset. When $\alpha_3 = 0$, the regularizer is not used. As $\alpha_3$ increases, the mask regularizer starts to work and improve the quality of the point-wise map. When $\beta_3$ is too large, the other terms, e.g., the descriptor-preservation term, make little contribution, and therefore the point-wise map degrades. We can see that within the range where the regularizers have a positive effect (e..g., between 0.1 and 5), the new mask (the red curve) uniformly outperforms the old mask (the green curve). This test provides empirical support that the new mask has a better performance than the old mask in general.
Fig.~\ref{fig:res:diffWeight:example} shows qualitative results with different weights of the regularizer term (using the old and new formulation resp.) for a TOSCA isometric pair.

We explored the performance of our regularizer by changing the value $\gamma$ in the definition of our mask. Namely, Fig.~\ref{fig:res:diffGamma:faust} shows the performance of the new mask (red sold curve) w.r.t. different choices of the parameter $\gamma$ across different datasets, where the performance of the old mask (blue dashed line) is added as a reference. The performance varies w.r.t. the choice of $\gamma$, but all of them are better than the old mask for the first three datasets, which shows that the general structure of the new mask outperforms the old mask. Note also that the optimal choice of $\gamma$ is larger for more isometric datasets, which confirms the intuition introduced earlier.

% Table~\ref{tb:res:coverage} shows the coverage of the point-wise map of the initialization without any refinement, with the old and the new mask regularizer, where the coverage is defined as the ratio between the area of the covered vertices and the total surface area of the target shape. We can see that, the new mask can improve the coverage of the point-wise map at the same time.

Finally, Table.~\ref{tb:res:failureRate} shows the failure rate of the initialization with the new mask compared to the old one. We note that in a small fraction of cases, our mask results in worse performance than original the Laplacian-based one. Such cases, however are rare and regardless of the dataset and quality measure, we achieve improvement in over 85\% of the cases.

%\input{tables/tb_AveCoverage.tex}
\input{tables/tb_failureRate.tex}

==> tables/tb_AveCoverage.tex <==
\begin{table}[!t]
\centering
\begin{tabular}{ccccc}
\hline
Mask & \begin{tabular}[c]{@{}c@{}}FAUST \\ Iso\end{tabular} & \begin{tabular}[c]{@{}c@{}}FAUST \\ nonIso\end{tabular} & \begin{tabular}[c]{@{}c@{}}TOSCA \\ Iso\end{tabular} & \begin{tabular}[c]{@{}c@{}}TOSCA \\ nonIso\end{tabular} \\ \hline
old & 44.9\% & 41.6\% & 39.05\% & 22.3\% \\
new & 49.7\% & 47.1\% & 40.48\% & 25.9\% \\ \hline
\end{tabular}
\caption{Average coverage rate of the initial maps with different masks.}
\label{tb:res:coverage}
\end{table}

==> tables/tb_AveErr_Summary.tex <==
\begin{table*}[!t]
\centering
\begin{tabular}{cclllllllll}
\hline
\multirow{2}{*}{Datasets} & \multirow{2}{*}{mask} & \multicolumn{3}{c|}{Initialization $(\times 10^{-3})$} & \multicolumn{3}{c|}{with ICP $(\times 10^{-3})$} & \multicolumn{3}{c}{with BCICP $(\times 10^{-3})$} \\ \cline{3-11} 
 &  & \multicolumn{1}{c}{per vtx} & \multicolumn{1}{c}{per map} & \multicolumn{1}{c|}{direct} & \multicolumn{1}{c}{per vtx} & \multicolumn{1}{c}{per map} & \multicolumn{1}{c|}{direct} & \multicolumn{1}{c}{per vtx} & \multicolumn{1}{c}{per map} & \multicolumn{1}{c}{direct} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}FAUST\\ Isometric\end{tabular}} & old & 37.74 & 65.14 & 65.83 & 27.82 & 43.20 & 43.32 & 23.41 & 32.22 & 34.67 \\
 & new & 31.31 & 46.48 & 46.86 & 25.56 & 35.63 & 35.63 & 22.11 & 30.38 & 30.38 \\
 & \multicolumn{1}{l}{Improv.} & 17.0\% & 28.7\% & \textbf{28.8\%} & 8.12\% & 17.5\% & \textbf{17.8\%} & 5.55\% & 5.71\% & \textbf{12.4\%} \\[6pt]
 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}FAUST\\ non-Isometric\end{tabular}} & old & 46.77 & 89.51 & 90.81 & 34.65 & 63.63 & 64.83 & 24.47 & 42.07 & 42.60 \\
 & new & 37.17 & 66.08 & 68.37 & 30.93 & 53.61 & 55.53 & 23.28 & 38.09 & 39.07 \\
 & \multicolumn{1}{l}{Improv.} & 20.5\% & 26.2\% & \textbf{24.7\%} & 10.7\% & 15.8\% & \textbf{14.4\%} & 4.86\% & 9.46\% & \textbf{8.29\%} \\[6pt]
 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}TOSCA\\ Isometric\end{tabular}} & old & 48.36 & 80.08 & 81.70 & 40.38 & 63.37 & 66.12 & 30.08 & 42.55 & 45.19 \\
 & new & 40.75 & 66.84 & 68.85 & 34.83 & 53.85 & 56.11 & 29.06 & 40.34 & 43.69 \\
 & \multicolumn{1}{l}{Improv.} & 15.7\% & 16.5\% & \textbf{15.7\%} & 13.7\% & 15.0\% & \textbf{15.1\%} & 3.39\% & 5.19\% & \textbf{3.32\%} \\[6pt]
 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}TOSCA\\ non-Isometric\end{tabular}} & old & 237.1 & 323.8 & 326.5 & 184.7 & 261.6 & 271.0 & 79.8 & 110.4 & 128.7 \\
 & new & 150.8 & 256.7 & 260.1 & 140.6 & 209.9 & 227.4 & 68.9 & 88.7 & 110.1 \\
 & \multicolumn{1}{l}{Improv.} & 36.4\% & 20.7\% & \textbf{20.3\%} & 23.9\% & 19.8\% & \textbf{16.1\%} & 13.7\% & 19.7\% & \textbf{14.5\%} \\[2pt] \hline
\end{tabular}
\caption{\textbf{Average accuracy and relative improvement.} For each of the four datasets, we compare the new mask with the old one w.r.t. three settings (initialization, with ICP refinement, and with BCICP refinement), and w.r.t. three measurements (per-vertex, per-map and direct error), where the parameters are kept the same in the comparison and the relative improvement is also reported as "Improv."}
\end{table*}





==> tables/tb_AveErr_Summary_new.tex <==
\begin{table*}[!t]
\centering
\begin{tabular}{cclllllllll}
\hline
\multirow{2}{*}{Datasets} & \multirow{2}{*}{mask} & \multicolumn{3}{c|}{Initialization $(\times 10^{-3})$} & \multicolumn{3}{c|}{with ICP $(\times 10^{-3})$} & \multicolumn{3}{c}{with BCICP $(\times 10^{-3})$} \\ \cline{3-11} 
 &  & \multicolumn{1}{c}{per vtx} & \multicolumn{1}{c}{per map} & \multicolumn{1}{c|}{direct} & \multicolumn{1}{c}{per vtx} & \multicolumn{1}{c}{per map} & \multicolumn{1}{c|}{direct} & \multicolumn{1}{c}{per vtx} & \multicolumn{1}{c}{per map} & \multicolumn{1}{c}{direct} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}FAUST\\ Isometric\end{tabular}} & old & 37.74 & 65.14 & 65.83 & 27.82 & 43.20 & 43.32 & 23.41 & 32.22 & 34.67 \\
 & new & 31.31 & 46.48 & 46.86 & 25.56 & 35.63 & 35.63 & 22.11 & 30.38 & 30.38 \\
 & \multicolumn{1}{l}{Improv.} & 17.0\% & 28.7\% & \textbf{28.8\%} & 8.12\% & 17.5\% & \textbf{17.8\%} & 5.55\% & 5.71\% & \textbf{12.4\%} \\[6pt]
 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}FAUST\\ non-Isometric\end{tabular}} & old & 46.77 & 89.51 & 90.81 & 34.65 & 63.63 & 64.83 & 24.47 & 42.07 & 42.60 \\
 & new & 37.17 & 66.08 & 68.37 & 30.93 & 53.61 & 55.53 & 23.28 & 38.09 & 39.07 \\
 & \multicolumn{1}{l}{Improv.} & 20.5\% & 26.2\% & \textbf{24.7\%} & 10.7\% & 15.8\% & \textbf{14.4\%} & 4.86\% & 9.46\% & \textbf{8.29\%} \\[6pt]
 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}TOSCA\\ Isometric\end{tabular}} & old & 48.36 & 80.08 & 81.70 & 40.38 & 63.37 & 66.12 & 30.08 & 42.55 & 45.19 \\
 & new & 40.75 & 66.84 & 68.85 & 34.83 & 53.85 & 56.11 & 29.06 & 40.34 & 43.69 \\
 & \multicolumn{1}{l}{Improv.} & 15.7\% & 16.5\% & \textbf{15.7\%} & 13.7\% & 15.0\% & \textbf{15.1\%} & 3.39\% & 5.19\% & \textbf{3.32\%} \\[6pt]
 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}TOSCA\\ non-Isometric\end{tabular}} & old & 237.7 & 324.9 & 326.6 & 186.2 & 267.1 & 275.2 & 79.8 & 111.0 & 123.3 \\
 & new & 149.2 & 254.7 & 258.1 & 141.1 & 213.3 & 230.2 & 68.6 & 78.7 & 91.1 \\
 & \multicolumn{1}{l}{Improv.} & 37.2\% & 21.6\% & \textbf{21.0\%} & 24.2\% & 20.1\% & \textbf{16.4\%} & 14.0\% & 29.1\% & \textbf{26.1\%} \\[2pt] \hline
\end{tabular}
\caption{Average accuracy and relative improvement. For each of the four datasets, we compare the new mask with the old one w.r.t. three settings (initialization, with ICP refinement, and with BCICP refinement), and w.r.t. three measurements (per-vertex, per-map and direct error), where the parameters are kept the same in the comparison and the relative improvement ("Improv.") is also reported.}
\label{tb:res:aveErr_summary}
\end{table*}





==> tables/tb_failureRate.tex <==
\begin{table}[!t]
\begin{tabular}{ccccc}
\hline
Measure & \begin{tabular}[c]{@{}c@{}}FAUST \\ Iso\end{tabular} & \begin{tabular}[c]{@{}c@{}}FAUST \\ nonIso\end{tabular} & \begin{tabular}[c]{@{}c@{}}TOSCA \\ Iso\end{tabular} & \begin{tabular}[c]{@{}c@{}}TOSCA \\ nonIso\end{tabular} \\ \hline
per-vertex & 11.5\% & 8.75\% & 10.7\% & 1.58\% \\
per-map & 11.5\% & 12.0\% & 13.0\% & 1.58\% \\
direct & 11.5\% & 13.0\% & 13.9\% & 2.63\% \\ \hline
\end{tabular}
\caption{Failure Rate. The table lists the percentage of the pairs where the new mask produces worse results than the old mask before any refinement.}
\label{tb:res:failureRate}
\end{table}
